MorphNLI: A Stepwise Approach to Natural Language Inference Using Text Morphing

We introduce MorphNLI, a modular step-by-step approach to natural language inference (NLI). When classifying the premise-hypothesis pairs into {entailment, contradiction, neutral}, we use a language model to generate the necessary edits to incrementally transform (i.e., morph) the premise into the hypothesis. Then, using an off-the-shelf NLI model we track how the entailment progresses with these atomic changes, aggregating these intermediate labels into a final output. We demonstrate the advantages of our proposed method particularly in realistic cross-domain settings, where our method always outperforms strong baselines with improvements up to 12.6% (relative). Further, our proposed approach is explainable as the atomic edits can be used to understand the overall NLI label.

==> tables/manual.tex <==
\begin{tabular}{lrr}
\hline
 \textbf{Model} & \textbf{SICK} & \textbf{MNLI} \\
\hline
\name\ expl. & \textbf{70.63} ($\pm$4.27) & 70.00 ($\pm$5.40) \\
GPT-4o expl. & 62.50 ($\pm$5.40) & \textbf {92.50} ($\pm$5.00) \\
Llama 3.1 8B expl. & 47.50 ($\pm$12.50) & 56.67 ($\pm$7.64) \\
\hline
Morphism only & 95.63 ($\pm$3.15) & 82.50 ($\pm$3.54)   \\
\hline
\end{tabular}
